Assuring and critical labels for relations between maximal consistent sets for interpretability logics

The notion of a critical successor [dJV90] has been central to almost all modal completeness proofs in interpretability logics. In this paper we shall work with an alternative notion, that of an assuring successor. As we shall see, this will enable more concisely formulated completeness proofs, both with respect to ordinary and generalised Veltman semantics. Due to their interesting theoretical properties, we will devote some space to the study of a particular kind of assuring labels, the so-called full labels and maximal labels.. After a general treatment of assuringness, we shall apply it to obtain certain completeness results. Namely, we give another proof of completeness of ILW w.r.t. ordinary semantics and of ILP w.r.t. generalised semantics.

==> sassuringJournal.tex <==
\section{Existence and labelling lemmata}\label{section:existenceAndLabeling}

So far, we have only been concerned with the nature and closure properties of the respective kind of labels. In this section we see how to guarantee the existence of informative labels. Furthermore, we shall see how labels can reflect the particularities of each interpretability logic so that in a sense they will pre-code the respective frame conditions.

\subsection{Existence of assuring successors}


\input{existenceJoint}

\label{sec:labellinglemmata}
\subsection{Labelling lemmata}

Labels accrue information about the role of MCSs and their successors. As it turns out, each particular logic affects this information accrual. The information accrual in the labels most often is so that, in a sense, it pre-codes the frame condition of the respective logic at the level of MCSs and this is reflected in so-called \emph{labelling lemmata}.

We will now include some labelling lemmata. Even though some of the proofs are not new (the ones that do not deal with fullness), we do include them here to illustrate the interaction between axiom schemata, frame conditions and labelling lemmata. As such, the material in this subsection comes largely from \cite{Bilkova-Goris-Joosten} and a more detailed exposition can be found in \cite{GorisBilkovaJoostenMikec:2020:ArXivLabels}.

\paragraph{The principle \principle{P}.}
Let us see how frame conditions locally impose requirements on MCSs, taking \extil{P} as the first example. 
The frame condition for \principle{P} is the following \cite{jovelt90}:
\[
wRw'RuS_w v \Rightarrow uS_{w'}v.
\]

The frame condition for \principle{P} imposes on MCSs the following:
\[
\Gamma \prec \Lambda \prec \Delta S_\Gamma \Sigma \Rightarrow \Delta S_{\Lambda}\Sigma.
\]
%%\cite{jovelt90}

When a \mcs $\Sigma\ni D$ is chosen witnessing a formula $C\rhd D\in\Gamma\prec\Delta\ni C$ we want to be able to find $\Gamma\prec\Sigma$ (and the same formulas are assured), but also $\Lambda\prec\Sigma$. Moreover, if $\Lambda\prec_T\Delta$, it should be possible to choose $\Sigma$ so that $\Lambda\prec_T\Sigma$. Only then it is consistent to draw the $\Delta S_\Lambda \Sigma$ arrow required by the frame condition, as depicted in Figure \ref{fig:framecondP}. The labelling lemma for \principle{P} tells us that this is possible.

\begin{lemma}\label{lemm:labp}
For logics containing ${\sf P}$ we have
$\Gamma\sassuring{S}\Lambda\sassuring{T}\Delta\Rightarrow\Gamma\sassuring{S\cup\boxdotset{T}{\Lambda}}\Delta$.
\end{lemma}

\begin{proof}
Suppose $\neg C\rhd\bigvee\neg S_i\vee\bigvee \neg A_j\vee\Diamond \neg A_j\in\Gamma$,
where $\Box A_j, A_j\in\boxdotset{T}{\Lambda}$.
Then $\neg C\rhd\bigvee\neg S_i\vee\bigvee \neg A_j\in\Gamma$ and thus
by ${\sf P}$ we obtain $\neg C\rhd\bigvee\neg S_i\vee\bigvee \neg A_j\in\Lambda$.
Since $\Gamma\sassuring{S}\Lambda$ we have $\Box\bigwedge S_i\in\Lambda$ so we 
obtain
$\neg C\rhd\bigvee \neg A_j\in\Lambda$. But for each $A_j$ we have 
$\neg A_j\rhd\bigvee\neg T_{jk}\in\Lambda$
and thus $\neg C\rhd\bigvee\neg T_{jk}\in\Lambda$. Since $\Lambda\prec_T\Delta$ we 
conclude
$C,\Box C\in\Delta$.
\end{proof}



In the case of P, a simpler labelling lemma can be used to ensure the frame condition locally, provided we consider the labels that are \emph{full} ($S$ a $\Gamma$-full label, and $T$ a $\Lambda$-full label).

\begin{lemma}\label{lemm:labfullp}
For logics containing ${\sf P}$ we have 
$$
\Gamma\sassuring{S}\Lambda\sassuring{T}\Delta\Rightarrow\Gamma\sassuring{T}\Delta.
$$
\end{lemma}

\begin{proof}
Assume $\Gamma\sassuring{S}\Lambda\sassuring{T}\Delta$, and $\neg C\rhd \bigvee \neg T_i \in\Gamma$. Then by ${\sf P}$ we know $\neg C\rhd \bigvee \neg T_i \in\Lambda$. Since $\Lambda\prec_T\Delta$ we conclude $C,\Box C\in\Delta$. 
\end{proof}

By $S$ being a $\Gamma$-full label, and by Lemma \ref{theorem:informationAccrualOverFullLabels}, we have that $\boxdotset{S}{\Gamma} \subseteq S \subseteq T$, thus Lemma \ref{lemm:labfullp} provides the same information as Lemma \ref{lemm:labp} (given full labels).

\paragraph{The principle \principle{M}.}
The frame condition for \principle{M} is the following \cite{jovelt90}:
\[
wRuS_w v Rz \Rightarrow uRz.
\]

The frame condition for \principle{M} imposes on MCSs the following:
\[
\Delta S_\Gamma \Sigma \prec \Omega \Rightarrow \Delta \prec\Omega
\]

and this is duly reflected in the corresponding labelling lemma:

\begin{lemma}\label{lemm:labm}
For logics containing \principle{M} we have $\Gamma \sassuring{S} \Delta 
\Rightarrow \Gamma \sassuring{S\cup \boxset{\emptyset}{\Delta}} \Delta$.
\end{lemma}

\begin{proof}
Assume that for some $\Box C_j \in \boxset{\emptyset}{\Delta}$ we have 
$(\neg A\rhd\bigvee \neg S_i \vee \bigvee \neg \Box C_j) \in \Gamma$.
By \principle{M},
$(\neg A \wedge \bigwedge \Box C_j \rhd \bigvee \neg S_i) \in \Gamma$,
Equivalently, $\neg (A \vee \neg \bigwedge \Box C_j \rhd \bigvee \neg S_i) \in \Gamma$.
whence $\boxdot (A \vee \neg \bigwedge \Box C_j) \in \Delta$.
As $\bigwedge \Box C_j \in \Delta$, we conclude
$A, \Box A \in \Delta$.
\end{proof}

\paragraph{The principle \principle{M_0}.}
The frame condition for \principle{M_0} is \cite{vis97}:
\[
wRuRxS_w v Rz \Rightarrow uRz,
\]




which imposes on MCSs that
\[
\Gamma \prec \Delta \prec \Delta' S_\Gamma \Sigma \prec \Omega \Rightarrow \Delta \prec \Omega.
\]

The corresponding labelling lemma is the following: 

\begin{lemma}\label{lemm:labmo}
For logics containing \principle{M_0} we have
$\Gamma \sassuring{S} \Delta \sucs \Delta' \Rightarrow 
\Gamma \sassuring{S \cup \boxset{\emptyset}{\Delta}} \Delta'$.
\end{lemma}

\begin{proof}
Suppose $\neg C\rhd\bigvee \neg S_i\vee\bigvee\Diamond \neg A_j\in\Gamma$,
where $\Box A_j\in\boxset{\emptyset}{\Delta}$.
By ${\sf M}_0$ we obtain $\Diamond \neg C\wedge\bigwedge\Box A_j\rhd\bigvee 
\neg S_i\in\Gamma$.
So, since $\Gamma\sassuring{S}\Delta$ and $\bigwedge\Box A_j\in\Delta$ we 
obtain $\Box C\in\Delta$ and thus $\Box C, C\in\Delta'$.
\end{proof}


\paragraph{The principle \principle{R}.}
Last we will look at a more complicated case of \extil{R}.

The frame condition for the principle \principle{R} is the following \cite{jogo11}.
\[
wRxRyS_wy'Rz\Rightarrow yS_xz.
\]

On \mcs, the condition imposes the following:
\[
\Gamma \prec \Lambda \prec \Delta S_\Gamma \Sigma \prec \Omega\Rightarrow \Delta S_\Lambda \Omega.
\]
and this is reflected in the corresponding labelling lemma:

\begin{lemma}\label{lemm:labeltrans}\label{lemm:labr}
For logics containing \principle{R} we have
$\Gamma \sassuring{S} \Lambda \sassuring{T} \Delta \Rightarrow 
\Gamma \sassuring{S \cup \boxset{T}{\Lambda}} \Delta$.
\end{lemma}

\begin{proof}
We consider $A$ such that for some $S_i \in S$ and 
some $\Box A_j \in \boxset{T}{\Lambda}$, we have
$(\neg A \rhd \bigvee \neg S_i \vee \bigvee \Diamond \neg A_j) \in \Gamma$.
By \principle{R} we obtain 
$(\neg (\neg A \rhd \bigvee \neg A_j)\rhd \bigvee \neg S_i)\in \Gamma$,
thus by $\Gamma \sassuring{S} \Lambda$ we get
$(\neg A \rhd \bigvee \neg A_j) \in \Lambda$.
As $(\neg A_j \rhd \bigvee \neg T_{kj})\in \Lambda$, also
$(\neg A \rhd \bigvee \neg T_{kj})\in \Lambda$. By 
$\Lambda \sassuring{T} \Delta$ we conclude $\boxdot A \in \Delta$.
\end{proof}

In the case of \principle{R}, a simpler labeling lemma can be used to ensure the frame condition locally if $T$ is $\Lambda$-full: 

\begin{lemma}\label{lemm:labfullr}
For logics containing \principle{R} we have 
$\Gamma \sassuring{S} \Lambda \sassuring{T} \Delta \Rightarrow\Gamma\sassuring{S \cup \Box T} \Delta$
\end{lemma}

\begin{proof}
Assume $\neg A\rhd \bigvee \neg S_i \vee \bigvee \neg\Box T_j \in \Gamma$. Then, by \principle{R}, we obtain $\neg(\neg A\rhd \bigvee \neg T_j)\rhd \bigvee\neg S_i \in \Gamma$ and by $\Gamma\sassuring{S}\Lambda$ we know $\boxdot(\neg A\rhd \bigvee \neg T_j)\in \Lambda$, and $\boxdot A\in \Delta$ as required.
\end{proof}

As before in the case of logics containing \principle{P} and Lemma \ref{lemm:labfullp}, this lemma ensures the frame condition locally provided the labels are full: for in this case $\boxdotset{T}{\Lambda}\subseteq T$ and therefore, because $T$ is a theory, $\boxset{T}{\Lambda}\subseteq \Box T$, and consequently $S\cup\boxset{T}{\Lambda}\subseteq S\cup\Box T$.
Thus sufficient information is carried by the composed label.




\paragraph{The principle \principle{W}.}
We state two existence lemmata for \extil{W}, a logic for which only second order frame properties are known (\cite{jogo11}, \cite{Mikec-Perkov-Vukovic-17}).\footnote{The property from \cite{Mikec-Perkov-Vukovic-17} is that for every $w$, $u$, $V$, if $u S_w V$, then there is $V' \subseteq V$ such that $uS_w V'$ and $\{ z : (\exists v \in V') vRz \}$ and $\{ z : z S_w V \}$ are disjoint (i.e., $R[V'] \cap S_w^{-1}[V] = \emptyset$).}


\begin{lemma}\label{lemm:wprobs}
Suppose $\neg(A\rhd B)\in\Gamma$ and $\Gamma$ is an \ilx-\mcs. There exists some \ilx-\mcs $\Delta$ with
$\Gamma\prec_{\{\Box\neg A,\neg B\}}\Delta$ and $A\in\Delta$.
\end{lemma}

\begin{proof}
Suppose for a contradiction that there is no such $\Delta$.
Then there are finitely many formulas $E_i$ such that $(\neg E_i\rhd \Diamond A\vee B)\in\Gamma$ and $A, \{E_i, \Box E_i\}_i \vdash\bot$. Let $E = \bigwedge_i E_i$. By \extil{} and maximal consistency we have $(\neg E\rhd \Diamond A\vee B)\in\Gamma$ and
$A, E, \Box E\vdash\bot$. Thus $\vdash A\rhd \neg E$.
Then $(A\rhd \Diamond A\vee B)\in\Gamma$ and by the principle $\principle{W}$ we have $A\rhd B\in\Gamma $.
The contradiction.
\end{proof}


\begin{lemma}\label{lemm:wdefies}
For logics containing \principle{W} we have that if
$B\rhd C \in \Gamma \sassuring{S} \Lambda \ni B$ then there exists
$\Delta$ (an \ilx-\mcs w.r.t.~the same logic \ilx) with
$\Gamma \sassuring{S\cup \{ \Box \neg B\}} \Delta \ni C, \Box \neg C$.
\end{lemma}

\begin{proof}
Suppose for a contradiction that no such $\Delta$ exists. Then
for some formula $A$ with 
$(\neg A \rhd \bigvee \neg S_i \vee \Diamond B) \in \Gamma$, we get
$C, \Box \neg C, A, \Box A \vdash \bot$, whence
$\vdash C\rhd \neg A$. Thus 
$B\rhd C \rhd \neg A \rhd \bigvee \neg S_i \vee \Diamond B \in \Gamma$.
By \principle{W}, $B \rhd \bigvee \neg S_i \in \Gamma$ which 
contradicts 
$\Gamma\sassuring{S} \Lambda \ni B$.
\end{proof}





%We propose the following slogan.
%\begin{quote} {\bf Slogan:} Every complete logic with a first order frame condition has its own labelling lemma. \end{quote}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%include P picture
\begin{figure}
    \centering
    % ILP
    \begin{minipage}[b]{0.47\textwidth} 
        \centering
        \input{fig_ilp}
        \caption{\footnotesize Ensuring frame condition for  ${\sf P}$}
        \label{fig:framecondP}
    \end{minipage}
    % ILM
    \begin{minipage}[b]{0.47\textwidth} 
        \centering
        \input{fig_ilm}
        \caption{\footnotesize Ensuring frame condition for  ${\sf M}$}
        \label{fig:framecondM}
    \end{minipage}
\end{figure}   
%%%%%%%%%%%%%%%%%%%%%%%%%%%




